Evaluating Small Language Models for News Summarization: Implications and Factors Influencing Performance

The increasing demand for efficient summarization tools in resource-constrained environments highlights the need for effective solutions. While large language models (LLMs) deliver superior summarization quality, their high computational resource requirements limit practical use applications. In contrast, small language models (SLMs) present a more accessible alternative, capable of real-time summarization on edge devices. However, their summarization capabilities and comparative performance against LLMs remain underexplored. This paper addresses this gap by presenting a comprehensive evaluation of 19 SLMs for news summarization across 2,000 news samples, focusing on relevance, coherence, factual consistency, and summary length. Our findings reveal significant variations in SLM performance, with top-performing models such as Phi3-Mini and Llama3.2-3B-Ins achieving results comparable to those of 70B LLMs while generating more concise summaries. Notably, SLMs are better suited for simple prompts, as overly complex prompts may lead to a decline in summary quality. Additionally, our analysis indicates that instruction tuning does not consistently enhance the news summarization capabilities of SLMs. This research not only contributes to the understanding of SLMs but also provides practical insights for researchers seeking efficient summarization solutions that balance performance and resource use.

==> ARR_version/01introduction.tex <==
\section{Introduction}
% \cite{zhang2024benchmarking} modify the figure to fig.

% 大模型

% text summarization for database or search engine optimization
% SEO
% Frontiers: Supporting Content Marketing with Natural Language Generation
% Text Summarization Techniques for Meta Description Generation in Process of Search Engine Optimization
% Design of optimal search engine using text summarization through artificial intelligence techniques
% https://wordlift.io/blog/en/text-summarization-in-seo/
% https://marketbrew.ai/a/text-summarization-seo#how-does-text-summarization-impact-the-readability-and-user-experience-of-a-website
%  Web-page classification through summarization. 
% DeepTitle -- Leveraging BERT to generate Search Engine Optimized Headlines
% Searching web documents using a summarization approach

% database
% Automatic Text Summarization Methods: A Comprehensive Review
% Querying a summary of database
% Text summarization in the biomedical domain: A systematic review of recent research
% https://www.frase.io/blog/20-applications-of-automatic-summarization-in-the-enterprise/

% IR
% Application of Text Summarization techniques to the Geographical Information Retrieval task

%金融预测
%搜索引擎优化
%

% Automatic text summarization is a classic problem in the field of natural language processing (NLP) with a wide range of applications~\cite{tam2015webtablesumm,2019soe,sharma2022database_summ}.

Automatic text summarization is a classic problem in the field of Natural Language Processing (NLP), with wide applications in areas such as search engine optimization~\cite{2019soe}, financial forecasting\cite{fintech}, and public sentiment analysis~\cite{twitter_news}. And the advent of large language models (LLMs) like GPT-3~\cite{NEURIPS2020_gpt3}, OPT~\cite{opt}, and Llama2~\cite{touvron2023llama2openfoundation} has revolutionized the field of text summarization. LLMs not only improve the summarization quality but also generate more flexible and coherent summaries than traditional text summarization models~\cite{luhn1958automatic, dong-etal-2018-banditsum, zhang-etal-2018-neural, t5, genest-lapalme-2012-fully}. \citet{zhang2024benchmarking} indicated that human evaluators show an equal preference for summaries generated by freelance writers and those produced by LLMs.


However, the hundreds of billions of parameters in LLMs require substantial computational and storage resources. For example, to efficiently deploy the Llama2-70B model at FP16 precision, we typically require two Nvidia A100 GPUs with 80GB of memory each. This means that only organizations with significant computing power can offer LLM services, raising concerns about service stability and data privacy. As a result, small language models (SLMs) have emerged as a potential alternative. They typically use a decoder-only architecture and have text generation capabilities similar to LLMs but with fewer than 4B parameters~\cite{azure2024phi,qwen,cai2024internlm2,abdin2024phi3,llama3.2}. They are designed to run efficiently on edge devices like smartphones and personal computers, making them more accessible.



% Despite their smaller size, SLMs have already achieved competitive performance by leveraging advanced training techniques and high-quality training data.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{ARR_version/fig/introduction_example.pdf}
    \caption{Comparison of news summaries by Phi3-Mini and LLMs. Phi3-Mini is comparable to LLMs with fewer words, highlighting the potential of SLMs.  }
    \label{fig:intro}
\end{figure}



% Using SLM instead of LLM for news summarization on the edge devices is a low-cost method that also protects user privacy. 

Due to the high demands for efficiency and data privacy in areas like financial forecasting and sentiment analysis, using SLMs for text summarization on the edge is quicker, safer, and more stable than relying on cloud-based LLMs. However, there is currently a lack of comprehensive works evaluating the capabilities of SLMs in text summarization. Titans~\cite{tiny_titan} evaluated the capabilities of SLMs in meeting summarization, but it did not include general-purpose SLMs, and the ROUGE metric~\cite{lin-2004-rouge} they used only reflects the quality in terms of relevance and is heavily influenced by the reference quality~\cite{zhang2024benchmarking}. \citet{lu2024smalllanguagemodelssurvey} conducted a broader evaluation of SLMs across various tasks but did not include text summarization, leaving a gap in understanding SLMs in this area.



% However, while several studies have demonstrated the strong text generation capabilities of SLMs, their specific abilities in the domain of news summarization remain underexplored. Tiny Titans~\cite{tiny_titan} evaluated the capabilities of SLMs in meeting summarization, but it did not include general-purpose SLMs, and the ROUGE metric~\cite{lin-2004-rouge} they used is heavily influenced by the reference quality and does not cover all aspects of the summary evaluation~\cite{zhang2024benchmarking}. \citet{lu2024smalllanguagemodelssurvey} conducted a broader evaluation of SLMs across various tasks but did not include news summarization, leaving a gap in understanding SLM in this area.


In this paper, we aim to conduct a comprehensive evaluation and analysis of SLMs for news summarization, a process that compresses news articles into shorter versions while preserving key information as shown in Figure~\ref{fig:intro}. We first benchmark 19 SLMs on 2,000 news samples, evaluating their performance based on relevance, coherence, factual consistency, and summary length. Despite notable differences among SLMs, we find that the best-performing ones can generate news summaries comparable in quality to LLMs, while producing shorter summaries. This makes SLMs a possible choice for real-time summarization tasks. And among all the SLMs we evaluated, Phi3-Mini and Llama3.2-3B-Ins perform the best. Furthermore, we explore the impact of prompt design and instruction tuning on the news summarization capabilities of SLMs.

% We also investigate the factors influencing the news summarization capabilities. Our findings indicate that prompt engineering has a limited impact on enhancing the summarization abilities, with even complex prompts potentially degrading model performance. Therefore, simple prompts are enough in practical applications. Furthermore, the effects of instruction tuning on SLMs vary significantly. The quality of summaries generated by the Llama3.2 series models shows a significant improvement after instruction tuning, which aligns with \citet{zhang2024benchmarking}'s conclusions. However, the summary quality of the Qwen2 and InternLM2 series models shows almost no change after instruction tuning. 


In summary, our contributions are as follows: 
\begin{itemize}
  
    \item We benchmark 19 SLMs on 2,000 news articles, finding that models like Phi3-Mini and Llama3.2-3B-Ins achieve performance comparable to 70B LLMs, with the advantage of producing shorter summaries. 
    
    \item Our experiments reveal that simple prompts outperform complex ones in SLM summarization, suggesting practical implications for prompt design.

    \item We find that instruction tuning has inconsistent effects on SLM performance, with significant improvements in models like Llama3.2 but minimal gains in others like Qwen2 and InternLM2.
    
\end{itemize}

The remainder of the paper is organized as follows: Section~\ref{sec:background} covers the background and related work, Section~\ref{sec:method} details the methodology employed in our evaluation, Section~\ref{sec:setup} introduces our experimental setup, Section~\ref{sec:benchmark} presents the benchmarking results of SLMs, Section~\ref{sec:factor} analyzes the influencing factors on SLM summarization, Section~\ref{sec:Verification} verifies our evaluation method, and Section~\ref{sec:conclusion} concludes with a summary of findings and future work.








% When evaluating the text summarization capabilities of LLMs, many existing works~\cite{laskar-etal-2023-systematic,goyal2022news} have found that while traditional models like Pegasus~\cite{pegasus} and Brio~\cite{brio} outperform LLMs on reference-based metrics such as ROUGE~\cite{lin-2004-rouge}, human evaluators often prefer the summaries generated by LLMs. Additionally, other studies~\cite{fabbri2021summeval,zhang2024benchmarking} have shown that reference-based metrics typically have a low correlation with human evaluations because of low-quality reference summaries. Although we can directly use human evaluation, the high financial cost prevents us from applying it to large-scale models and datasets. Existing research~\cite{fabbri2021summeval} also found significant differences in the quality of human annotators, leading to substantial fluctuations in inter-annotator agreement. Recently, some works~\cite{goyal2022news,kendeer,gao2023human-like,liu2023benchmarking,wang2023chatgpt} have explored using LLMs as evaluators and found they correlate highly with the human evaluation. However, this approach also faces the high cost of LLM API usage~\cite{laskar-etal-2023-systematic} and fair issues~\cite{not-yet}.


% Therefore, this paper aims to evaluate the text summarization capabilities of SLMs using low-cost and effective metrics and to analyze the factors influencing the text summarization performance of SLMs. First, in order to improve the consistency between reference-based evaluation and human evaluation, we use LLMs to generate high-quality reference summaries. Our experiments demonstrate that high-quality references can increase the Kendall correlation coefficient with human evaluations from 0.43 to 0.74 in summary relevance, closing to the consistency between different human evaluators. Then, We evaluate several SLMs, including TinyLlama~\cite{zhang2024tinyllama}, the GPT-Neo series~\cite{gpt-neo-paper}, the Qwen2 series~\cite{qwen}, the Phi series~\cite{microsoft2023phi2,abdin2024phi3}, and others, from four perspectives: relevance, coherence, factual consistency, and summary length. Phi3-Mini can perform well across all dimensions, sometimes surpassing 7B LLMs. Finally, we study the impact of prompt design, instruction tuning, model size, and training data on the text summarization capabilities of SLMs. Among these factors, model size and the quality of training data had the most significant influence, while the effects of the other factors were relatively limited.



==> ARR_version/02background.tex <==
\section{Background and Related Work}
\label{sec:background}
% \subsection{Text Data Summarization}
% % Text summarization is a basic task in NLP domains that aims to compress original articles into a few sentences while retaining essential information and meaning. Overall, text summarization can be divided into extractive summarization and abstractive summarization.


% Text data summarization significantly enhances the efficiency of data processing, storing, and retrieving by extracting and generating concise summaries. For example, it helps search engines better determine the relevance between queries and results~\cite{MarketBrew2024SEO}. Overall, text summarization can be divided into extractive summarization and abstractive summarization.

% % Over the past few years, various approaches have been developed to enhance the performance of news summarization~\cite{zhou-etal-2018-neural-document,dong-etal-2018-banditsum,zhang-etal-2018-neural,t5,pegasus,brio,lewis-etal-2020-bart}. 

% % \subsubsection{Extractive Summarization}
% Extractive summarization is selecting the most relevant sentences from the original text to form a summary. This can ensure the relevance and faithfulness of the summary but may result in a lack of coherence or some redundant information. Early methods often use statistical or graph-based approaches to measure sentence importance. Luhn~\cite{luhn1958automatic} proposed a method based on word frequency statistics to select the most important sentences from a text. And TextRank~\cite{mihalcea2004textrank} is a graph-based ranking algorithm that represents the text as a graph, where nodes represent basic units of the text (such as words or sentences), and edges represent relationships between these units. Through the structure of the graph and the strength of connections between nodes, the TextRank algorithm can evaluate the importance of each node. BanditSum~\cite{dong-etal-2018-banditsum} addressed sentence selection by framing it as a contextual bandit problem. With the development of word embeddings~\cite{mikolov2013word2vec}, many works have started using semantic information to select sentences. For instance, NEUSUM~\cite{zhou-etal-2018-neural-document} and LATENT~\cite{zhang-etal-2018-neural} all encode
% the sentences and documents. Recently, some efforts have also considered improving extractive summarization based on LLMs. LaMSUM~\cite{chhikara2024lamsum} is a multi-level framework or extractive summarization. Parmar et al.~\cite{parmar2024enhancingcoherenceextractivesummarization} improved the extractive summarization capabilities of LLMs through fine-tuning training.


% Abstractive summarization, on the other hand, generates new sentences that cover the key information of the source text. Although this method offers better readability than extractive summarization, it faces challenges in maintaining the relevance and faithfulness of the summary. Initially, abstractive summarization often relies on techniques such as concatenation~\cite{jing2000cut} and rule matching~\cite{genest-lapalme-2012-fully} to generate summaries. With the rise of the Transformer architecture and pre-trained models, some efforts have achieved promising results. Pointer Generator~\cite{see-etal-2017-get}, based on the encoder-decoder architecture, can flexibly copy words from the source text or generate new words, thereby enhancing the accuracy and readability of summaries. T5~\cite{t5} is a pre-trained model that unifies all text processing tasks into a text-to-text format. Through pre-training on large-scale data and multi-task learning, it improves the performance of abstractive summarization. Pegasus~\cite{pegasus} is a pre-trained model designed for text summarization. It achieves pre-training by simulating the deletion of sentences to generate summaries. Brio~\cite{brio} improves summary quality by incorporating evaluation models during training. Recent works~\cite{dead_summarization,zhang2024benchmarking} indicate that LLMs have surpassed traditional sequence-to-sequence neural networks in abstractive summarization and can even achieve human-level performance.


% algo work
% evaluation work
% system level
\subsection{Small Language Model}
% Although LLMs have surpassed traditional neural network models in many NLP tasks, their enormous parameter sizes and computational requirements make them nearly impractical for consumer-grade devices. Additionally, using commercial APIs raises issues related to cost and privacy protection. Therefore, Some studies such as TinyLalma~\cite{zhang2024tinyllama}, Phi2~\cite{microsoft2023phi2}, etc. aim to achieve LLM-like text generation capabilities using smaller models and less data, which we call small language models (SLM). There is no clear definition specifying the parameter count for SLMs. Generally, SLMs are considered capable of running on mobile devices. Therefore, in this paper, we primarily explore models smaller than 8GB in FP16 precision, equivalent to fewer than 4B parameters.


Small language models (SLMs) typically refer to models with fewer parameters and a smaller computational footprint compared to larger LLMs. These include general-purpose and specialized models that can typically be deployed for inference on edge devices, such as mobile phones and PCs. With the increasing focus on general-purpose SLMs, this paper centers on their evaluation, hereafter referred to simply as SLMs. Structurally, both SLMs and LLMs consist of stacked decoder layers from the transformer architecture~\cite{attention_all_you_need}, generating output autoregressively. However, SLMs have fewer decoder layers, attention heads, and smaller hidden dimensions, and they are trained on smaller, high-quality datasets. There is no clear definition specifying the parameter count for SLMs, but they are generally considered capable of running on consumer-grade devices. This paper focuses on models smaller than 8GB in FP16 precision, corresponding to fewer than 4B parameters.

% Like LLMs, SLMs also have instruction-following capabilities. Thus, when using SLMs for text summarization, we need to input the original text along with prompts related to the summary. The model then generates the briefly summary. Fig~\ref{fig:diff_prompt_example} shows some prompt templates. By modifying the prompts, we can obtain summaries in different styles, making SLMs more flexible than traditional text summarization models.


%可能需要增加内容
\subsection{Text Summarization Evaluation}
Currently, there are many works evaluating models for text summary generation, covering aspects such as relevance, coherence, and factual consistency~\cite{huang-etal-2020-achieved,fabbri2021summeval,dead_summarization,zhang2024benchmarking,liu2023benchmarking}. \citet{huang-etal-2020-achieved} used ROUGE and human evaluation to evaluate 10 representative summarization models, finding that extractive summarizers performed better in human evaluations. In the Summeval benchmark~\cite{fabbri2021summeval}, the authors analyzed existing metrics and used human evaluation methods to assess 23 models. \citet{dead_summarization} evaluated the text summarization performance of LLMs and found that they were more favored by evaluators. \citet{zhang2024benchmarking} used human evaluation to evaluate LLMs, discovering that instruction tuning had a greater impact on performance than model size. INSTRUSUM~\cite{liu2023benchmarking} evaluated instruction controllable summarization of LLMs and found them still unsatisfactory in summarizing text based on complex instructions.

Although SLMs have shown strong capabilities, comprehensive comparisons of their text summarization abilities are still lacking. Tiny Titans~\cite{tiny_titan} assessed the summarization performance of SLMs in meeting summarization, but it focused only on older models, excluding newer series like the Phi3 and Llama3. Moreover, its evaluation was limited to the ROUGE metric, which is not sufficiently comprehensive. While \citet{lu2024smalllanguagemodelssurvey} evaluated SLMs across various tasks, news summarization was notably absent. Therefore, this paper aims to provide a thorough evaluation of SLM performance in news summarization.




% 没有完整定义
% sml
%system level
% news summarization
